An Automatic Learning Rate Schedule Algorithm for Achieving Faster Convergence and Steeper Descent

The delta-bar-delta algorithm is recognized as a learning rate adaptation technique that enhances the convergence speed of the training process in optimization by dynamically scheduling the learning rate based on the difference between the current and previous weight updates. While this algorithm has demonstrated strong competitiveness in full data optimization when compared to other state-of-the-art algorithms like Adam and SGD, it may encounter convergence issues in mini-batch optimization scenarios due to the presence of noisy gradients. In this study, we thoroughly investigate the convergence behavior of the delta-bar-delta algorithm in real-world neural network optimization. To address any potential convergence challenges, we propose a novel approach called RDBD (Regrettable Delta-Bar-Delta). Our approach allows for prompt correction of biased learning rate adjustments and ensures the convergence of the optimization process. Furthermore, we demonstrate that RDBD can be seamlessly integrated with any optimization algorithm and significantly improve the convergence speed. By conducting extensive experiments and evaluations, we validate the effectiveness and efficiency of our proposed RDBD approach. The results showcase its capability to overcome convergence issues in mini-batch optimization and its potential to enhance the convergence speed of various optimization algorithms. This research contributes to the advancement of optimization techniques in neural network training, providing practitioners with a reliable automatic learning rate scheduler for achieving faster convergence and improved optimization outcomes.

==> preli.tex <==


% \begin{assumption}\label{ass:upper_bound_x_norm}
%     Let $f(x)$ be define as Definition~\ref{def:f}, we denote that $x^* = \arg \min_{x} f(x)$, for any step $t$ as a integer, we assume that 
%     \begin{align*}
%         \| x_t - x^* \| \leq D
%     \end{align*}
%     where $D > 0$ is a scalar.
% \end{assumption}

% \begin{definition}
%     We now define the regret in optimization problem. We run $T$ steps of optimization, we define
%     \begin{align*}
%         R(T) := \sum_{t=1}^T f(x_t) - \sum_{t=1}^T \min_{x} f(x)
%     \end{align*}
% \end{definition}

% \section{Convergence of of SGD}

% \subsection{Definitions}

% \begin{definition}\label{def:sgd}
%     We run SGD on with loss function $f$, at $t$ step, we optimize
%     \begin{align*}
%         x_{t+1} = x_{t} - \alpha \nabla f_{\xi_t}(x_{t})
%     \end{align*}
% \end{definition}

% \begin{definition}\label{def:regret_sgd}
%     We run SGD on with loss function $f$ for $T$ step, we define
%     \begin{align*}
%         R_{\rm SGD}(T) := \sum_{t=1}^T f(x_t) - \sum_{t=1}^T \min_{x} f(x)
%     \end{align*}
% \end{definition}

% \subsection{Upper Bound on Regret of SGD}

% \begin{lemma}\label{lem:descnt_sgd}
%     We run SGD at $t$ step, let $f(x)$ be define as Definition~\ref{def:f}, let $R_{\rm SGD}(T)$ be defined as Definition~\ref{def:regret_sgd}, we have
%     \begin{align*}
%         R_{\rm SGD}(T) \leq ???
%     \end{align*}
% \end{lemma}

% \begin{proof}
%     We have
%     \begin{align}\label{eq:expansion_upper_bound_R_sgd}
%         R_{\rm SGD}(T)
%         = & ~ \sum_{t=1}^T f(x_t) - \sum_{t=1}^T \min_{x} f(x) \notag \\
%         = & ~ \sum_{t=1}^T (f(x_t) - \min_{x} f(x)) \notag \\
%         \leq  & ~ \sum_{t=1}^T (\nabla f(x_t)^\top (x_t - x^*) + \frac{1}{2}L \| x_t - x^* \|_2^2 ) 
%     \end{align}
%     where the first equality follows from Definition~\ref{def:regret_sgd}, the second equality follows from simple algebra, the third inequality follows from Corollary~\ref{cor:lipschitz}.

%     Next, we expand $\| x_{t+1} - x^* \|_2^2$, we have
%     \begin{align}\label{eq:expansion_x*_xt}
%         \| x_{t+1} - x^* \|_2^2 
%         = & ~ \| x_{t} - x^* - \alpha \nabla f_{\xi_t}(x_t) \|_2^2 \notag \\
%         = & ~ \| x_{t} - x^* \|_2^2 - 2\alpha \langle f_{\xi_t}(x_t), x_{t} - x^* \rangle + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2
%     \end{align}
%     where the first equality follows from Definition~\ref{def:sgd}, the second equality follows from simple algebra.

%     Then we have
%     \begin{align*}
%         R_{\rm SGD}(T)
%         \leq  & ~ \sum_{t=1}^T (\nabla f(x_t)^\top (x_t - x^*) + \frac{1}{2}L \| x_t - x^* \|_2^2 ) \\
%         = & ~ \sum_{t=1}^T (\frac{1}{2\alpha}(\| x_{t} - x^* \|_2^2 - \| x_{t+1} - x^* \|_2^2 + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2) + \frac{1}{2}L \| x_t - x^* \|_2^2 ) \\
%         \leq & ~ \sum_{t=1}^T (\frac{1}{2\alpha}(\| x_{t} - x^* \|_2^2 + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2) + \frac{1}{2}L \| x_t - x^* \|_2^2 ) \\
%         \leq & ~ \sum_{t=1}^T (\frac{1}{2\alpha}(D^2 + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2) + \frac{1}{2}L D^2) \\
%         \leq & ~ \sum_{t=1}^T (\frac{1}{2\alpha}(D^2 + \alpha^2 \sigma^2) + \frac{1}{2}L D^2) \\
%         = & ~ \sum_{t=1}^T (\frac{1}{2\alpha}D^2 + \frac{1}{2\alpha} \sigma^2) + \frac{1}{2}L D^2)
%     \end{align*}
%     where the first inequality follows from Eq.~\eqref{eq:expansion_upper_bound_R_sgd}, the second equality follows from Eq.~\eqref{eq:expansion_x*_xt}, the third inequality follows from $\| x_{t+1} - x^* \|_2^2 > 0$ and simple algebra, the fourth inequality follows from Assumption~\ref{ass:upper_bound_x_norm}, the fifth inequality follows from Assumption~\ref{ass:upper_bound_grad_f}.

%     % \begin{align*}
%     %     R_{\rm SGD}(T)
%     %     \leq & ~ \sum_{t=1}^T \frac{1}{2}L \| x_t - x^* \|_2^2  \\
%     %     = & ~ \sum_{t=1}^T \frac{1}{2}L \| x_t - x_{t-1} + x_{t-1} - x^* \|_2^2  \\
%     %     = & ~ \sum_{t=1}^T \frac{1}{2}L ( \| x_t - x_{t-1} \|_2^2 + 2\langle x_t - x_{t-1}, x_{t-1} - x^* \rangle + \| x_{t-1} - x^* \|_2^2 ) \\
%     % \end{align*}
% \end{proof}

% \subsection{Minimizing Guarantee of SGD}

% \begin{theorem}
%     Suppose $f$ has $\sigma$-bounded gradients, let $\alpha_t = \alpha = c / \sqrt{T}$, where $c = \sqrt{\frac{2( f(x) - f(x^*) )}{L\sigma^2}}$, and $x^*$ is an optimal solution to Definition~\ref{def:sgd}. Then, the iterates of SGD satisfy
%     \begin{align*}
%         \min_{0 \leq t \leq T-1} \E[\| \nabla f(x_t) \|^2] \leq \sqrt{\frac{2( f(x) - f(x^*) )L}{T}\sigma}
%     \end{align*}
% \end{theorem}

% \subsection{Adam}

% \subsubsection{Descent Lemma of Adam}

% \subsubsection{Minimizing Guarantee of Adam}



% \begin{definition}\label{def:g}
%     At $t$ step, we have loss function $f(x)$ with parameters $x$, we run SGD with learning rate $\alpha$, we define
%     \begin{align*}
%         g(x_t, \alpha) = f(x_t - \alpha \nabla f(x_t))
%     \end{align*}
% \end{definition}

% \begin{definition}\label{def:alpha_t}
%     At $t$ step, we have loss function $f(x)$ with parameters $x$, we run SGD with learning rate $\alpha_t$, we define $\alpha_{t-1}$ is the learning rate of $t-1$ step optimization, and $\alpha_{t} = \alpha_{t-1} - \eta \nabla_{\alpha_{t-1}} g_{\xi_t}(x_{t-1}, \alpha_{t-1})$
% \end{definition}

\subsection{Computation Result of \texorpdfstring{$\nabla_\alpha g(x_t, \alpha)$}{}}

\begin{lemma}\label{lem:grad_g}
    Let $g(\alpha)$ be define as Definition~\ref{def:g}, we have
    \begin{align*}
        \nabla_\alpha g(x_t, \alpha) = \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f(x_t) \rangle 
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \nabla_\alpha g(x_t, \alpha)
        = & ~ \nabla_\alpha f(x_t - \alpha \nabla f(x_t)) \\
        = & ~ \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla_\alpha (x _t - \alpha \nabla f(x_t)) \rangle \\
        = & ~ \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f(x_t) \rangle 
    \end{align*}
    where the first equality follows from Definition~\ref{def:g}, the second and third equalities follows from simple differential rules.
\end{proof}

\subsection{Lipschitz Property for \texorpdfstring{$\nabla_\alpha g(x_t, \alpha)$}{}}

\begin{lemma}\label{lem:g_lipshcitz}
    If $f(x)$ is Lipschitz-smooth with constant $L$, let $g(\alpha)$ be defined as Definition~\ref{def:g}, we have
    \begin{align*}
        | \nabla g(x_t, \alpha) - \nabla g(x_t, \alpha') | \leq L \sigma^2 | \alpha - \alpha' |
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        | \nabla g(x_t, \alpha) - \nabla g(x_t, \alpha') |
        = & ~ | \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f_(x_t) \rangle - \langle \nabla f(x_{t} - \alpha' \nabla f(x_t)),  \nabla  f(x_t) \rangle | \\ 
        \leq & ~ \| \nabla f(x_{t} - \alpha \nabla f(x_t)) -  \nabla f(x_{t} - \alpha' \nabla f(x_t)) \|_2 \cdot \| \nabla  f(x_t) \|_2 \\ 
        \leq & ~ \sigma \| \nabla f(x_{t} - \alpha \nabla f(x_t)) -  \nabla f(x_{t} - \alpha' \nabla f(x_t)) \|_2 \\ 
        \leq & ~ L \sigma \| (x_{t} - \alpha \nabla f(x_t)) - (x_{t} - \alpha' \nabla f(x_t)) \|_2 \\ 
        = & ~ L \sigma \| \alpha \nabla f(x_t) - \alpha' \nabla f(x_t) \|_2 \\ 
        \leq & ~ L \sigma | \alpha - \alpha' | \cdot \| \nabla f(x_t) \|_2 \\ 
        \leq & ~ L \sigma^2 | \alpha - \alpha' |
    \end{align*}
    where the first equality follows from Lemma~\ref{lem:grad_g}, the second inequality follows from Cauchy–Schwarz inequality, the third inequality follows from Assumption~\ref{ass:upper_bound_grad_f}, the fourth inequality follows from Assumption~\ref{ass:lipschitz}, the fifth equality follows from simple algebra, the sixth inequality follows from Cauchy–Schwarz inequality, the seventh inequality follows from Assumption~\ref{ass:upper_bound_grad_f}.
\end{proof}

\begin{lemma}\label{lem:cor_g_lipschitz}
    Since Lemma~\ref{lem:g_lipshcitz}, we have
    \begin{align*}
        g(x_t, \alpha) - ( g(x_t, \alpha') + \nabla_\alpha g(x_t, \alpha) (\alpha - \alpha') ) \leq \frac{1}{2} L \sigma^2 | \alpha - \alpha' |^2
    \end{align*}
\end{lemma}

\begin{proof}
    This proof follows from Corollary~\ref{cor:lipschitz} and Lemma~\ref{lem:g_lipshcitz}.
\end{proof}

\subsection{Upper Bound on \texorpdfstring{$\nabla_\alpha g(x_t, \alpha)$}{}}

\begin{lemma}
    Let $g(x_t, \alpha)$ be define as Definition~\ref{def:g}, we have
    \begin{align*}
        | \nabla_\alpha g(x_t, \alpha) | \leq \sigma^2
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        | \nabla_\alpha g(x_t, \alpha) |
        = & ~ | \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f(x_t) \rangle | \\
        \leq & ~ \| \nabla f(x_{t} - \alpha \nabla f(x_t)) \|_2 \cdot \| \nabla  f(x_t) \|_2 \\
        \leq & ~ \| \nabla f(x_{t} - \alpha \nabla f(x_t)) \|_2 \cdot \sigma \\
        \leq & ~ \sigma^2
    \end{align*}
    where the first equality follows from Lemma~\ref{lem:grad_g}, the second inequality follows from Cauchy–Schwarz inequality, the third and fourth inequalities follow from Assumption~\ref{ass:upper_bound_grad_f}.
\end{proof}

\subsection{Lower Bound on \texorpdfstring{$\nabla_\alpha g(x_t, \alpha)$}{}}

\begin{lemma}\label{lem:lower_bound_g}
    Let $g(x_t, \alpha)$ be define as Definition~\ref{def:g}, we have
    \begin{align*}
        \nabla_\alpha g(x_t, \alpha) \geq 0
    \end{align*}
\end{lemma}

\begin{proof}
    % We have
    % \begin{align*}
    %     | \nabla_\alpha g(x_t, \alpha) |
    %     = & ~ | \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f(x_t) \rangle | \\
    %     = & ~ | \nabla f(x_{t} - \alpha \nabla f(x_t))^\top  \nabla  f(x_t) | \\
    %     \geq 0
    % \end{align*}
    % where the first equality follows from Lemma~\ref{lem:grad_g}, the second equality follows from simple algebra, the third inequality follows from Assumption~\ref{ass:lower_bound_inner_product_grad}.

    % We have
    % \begin{align*}
    %     \nabla_\alpha g(x_t, \alpha)
    %     = & ~ \langle \nabla f(x_{t} - \alpha \nabla f(x_t)),  \nabla  f(x_t) \rangle \\
    %     = & ~ \langle \nabla f(x_{t+1}), \nabla  f(x_t) \rangle \\
    %     = & ~ \frac{1}{\alpha} \langle \nabla f(x_{t+1}), x_t - x_{t+1} \rangle \\
    %     \geq & ~ \frac{1}{\alpha} ( f(x_{t}) - f(x_{t+1}) - \frac{1}{2} L \| \alpha \nabla f(x_t) \|_2^2 )
    % \end{align*}
    % where the first equality follows from Lemma~\ref{lem:grad_g}, the second and third equalities follows from $x_{t+1} = x_t - \alpha \nabla f(x_t)$, the fourth inequality follows from Corollary~\ref{cor:lipschitz}.

    We expand $\| x_{t+1} - x_{t-1} \|_2^2$, we have
    \begin{align}\label{eq:expansion_x_t+1-x_t-1}
        \| x_{t+1} - x_{t-1} \|_2^2
        = & ~ \| x_{t} - x_{t-1} - \alpha \nabla f_{\xi_t}(x_t) \|_2^2 \notag \\
        = & ~ \| x_{t} - x_{t-1} \|_2^2 - 2\alpha \langle \nabla f_{\xi_t}(x_t), x_{t} - x_{t-1} \rangle + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2
    \end{align}
    where the first equality follows from Definition~\ref{def:sgd}, the second equality follows from simple algebra.

    Then we have
    \begin{align*}
        \langle \nabla f_{\xi_t}(x_t), x_{t} - x_{t-1} \rangle
        = & ~ \frac{1}{2\alpha}( \| x_{t} - x_{t-1} \|_2^2 - \| x_{t+1} - x_{t-1} \|_2^2 + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2 ) \\
        = & ~ \frac{1}{2\alpha}( \| x_{t} - x_{t-1} \|_2^2 - \| x_{t+1} - x_t + x_t - x_{t-1} \|_2^2 + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2 ) \\
        % \geq & ~ \| x_{t} - x_{t-1} \|_2^2 - D + \| \alpha \nabla f_{\xi_t}(x_t) \|_2^2 \\
    \end{align*}
    where this equality follows from Eq.~\eqref{eq:expansion_x_t+1-x_t-1}.

    We take the expactation, we can show that
    \begin{align*}
        \E[\langle \nabla f_{\xi_t}(x_t), x_{t} - x_{t-1} \rangle]
        = & ~ \E[\langle \nabla f_{\xi_t}(x_t), \alpha \nabla f_{\xi_{t-1}}(x_{t-1}) \rangle] \\
        = & ~ \langle \nabla f(x_t), \alpha \nabla f(x_{t-1}) \rangle
    \end{align*}

    % Follows Lemma~\ref{lem:descnt_sgd}, we let $\gamma := (\alpha - \eta \nabla f_{\xi_t}(x_t)^\top f_{\xi_{t-1}}(x_{t-1}))$
    % \begin{align*}
    %     f(x_{t+1}) \leq f(x_t) + (\frac{1}{2}L \gamma^2 - \gamma)  \E[ \| \nabla f(x_t) \|_2^2]
    % \end{align*}
\end{proof}

\subsection{Main Result}

\begin{lemma}
    \begin{align*}
        g(x_t, \alpha_{t}) < g(x_t, \alpha_{t-1})
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align}\label{eq:descent}
        g(x_t, \alpha_{t})
        \leq & ~ g(x_t, \alpha_{t-1}) + \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) (\alpha_{t} - \alpha_{t-1}) + \frac{1}{2} L \sigma^2 | \alpha_{t} - \alpha_{t-1} |^2 \notag \\
        = & ~ g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) \notag \\
        & ~ + \frac{1}{2} L \sigma^2 | \eta \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) |^2 \notag \\
        = & ~ g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) \notag \\
        & ~ + \frac{1}{2} L \sigma^2 \eta^2 | \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) |^2
    \end{align}
    where the first inequality follows from Lemma~\ref{lem:cor_g_lipschitz}, the second equality follows from Definition~\ref{def:alpha_t}, the third step follows from simple algebra and $\eta \geq 0$.

    Then we take expectation, we have
    \begin{align*}
        \E[g(\alpha_{t+1})]
        \leq & ~ \E[g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) \\
        & ~ + \frac{1}{2} L \sigma^2 \eta^2 | \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) |^2] \\
        = & ~ g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \E[\nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1})] \\
        & ~ + \frac{1}{2} L \sigma^2 \eta^2 \E[| \nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1}) |^2] \\
        = & ~ g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) \\
        & ~ + \frac{1}{2} L \sigma^2 \eta^2 | \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) |^2 \\
        \leq & ~ g(x_t, \alpha_{t-1}) - \eta \nabla_{\alpha_{t-1}} g(x_t, \alpha_{t-1}) \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) \\
        & ~ + \frac{1}{2} L \sigma^2 \eta^2 | \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) |^2 \cdot | \nabla_{\alpha_{t-1}} g(x_{t}, \alpha_{t-1}) |^2 \\
        = & ~ g(x_t, \alpha_{t-1}) + (- \eta + \frac{1}{2} L \sigma^2 \eta^2 \cdot | \nabla_{\alpha_{t-1}} g(x_{t}, \alpha_{t-1}) | \cdot  \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) | ) \\
        & ~ \cdot | \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) | \cdot | \nabla_{\alpha_{t-1}} g(x_{t}, \alpha_{t-1}) | \\
        \leq & ~ g(x_t, \alpha_{t-1}) + (- \eta + \frac{1}{2} L \sigma^6 \eta^2)  \cdot | \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_{t-1}) | \cdot | \nabla_{\alpha_{t-1}} g(x_{t}, \alpha_{t-1}) |
    \end{align*}
    where the first inequality follows from Eq.~\eqref{eq:descent}, the second inequality follows from simple algebra, the third equality follows from $\E[\nabla_{\alpha_{t-1}} g_{\xi_{t-1}}(x_{t-1}, \alpha_{t-1})] = \nabla_{\alpha_{t-1}} g(x_{t-1}, \alpha_t)$, the fourth inequality follows from $| \nabla_{\alpha_{t-1}} g(x_{t}, \alpha_{t-1}) |^2 \geq 0$, the fifth equality follows from Lemma~\ref{lem:lower_bound_g} and simple algebra.

    Since it's easy to show that when $\eta < \frac{2}{L \sigma^6}$, we have
    \begin{align*}
        g(\alpha_{t+1}) < g(\alpha_t)
    \end{align*}
    where this inequality follows from simple algebra.
\end{proof}

\section{Minimizing Guarantee of AdaLR}

\begin{lemma}
    We have
\end{lemma}

\begin{proof}
    Follows Lemma~\ref{lem:descnt_sgd}, we let $\gamma := (\alpha - \eta \nabla f_{\xi_t}(x_t)^\top f_{\xi_{t-1}}(x_{t-1}))$
    \begin{align*}
        f(x_{t+1}) \leq f(x_t) + (\frac{1}{2}L \gamma^2 - \gamma)  \E[ \| \nabla f(x_t) \|_2^2]
    \end{align*}
\end{proof}
